Equicontinuity, Transitivity and Sensitivity: the Auslander-Yorke Dichotomy Revisited

We discuss topological equicontinuity and even continuity in dynamical systems. In doing so we provide a classification of topologically transitive dynamical systems in terms of equicontinuity pairs, give a generalisation of the Auslander-Yorke Dichotomy for minimal systems and show there exists a transitive system with an even continuity pair but no equicontinuity point. We define what it means for a system to be eventually sensitive; we give a dichotomy for transitive dynamical systems in relation to eventual sensitivity. Along the way we define a property called splitting and discuss its relation to some existing notions of chaos.

==> EqAndChaos/0.1Continuity.tex <==
\section{Continuous functions}

The material in this section is fairly stand-alone, however it will help us generalise some results to Hausdorff spaces (rather than compact Hausdorff spaces).\footnote{Please note: The definitions and results in this section are my own; insofar as I have come up with them alone and have not seen them elsewhere. Although usually this would go without saying, I include this statement because the ideas in this section seem so `natural' that it would almost seem strange if no one else had already conceived of them.}

\begin{definition} A function $f \colon X \to Y$ is said to be $T_1$ continuous at $x \in X$ if for any open cover $\mathcal{U}$ of $Y$ there exists an open cover $\mathcal{V}$ of $X$ such that for any $y \in X$, if there exists $V \in \mathcal{V}$ with $x,y \in V$ then there exists $U \in \mathcal{U}$ with $f(x),f(y) \in U$.

We say $f$ is $T_1$ continuous if it is $T_1$ continuous at all $x \in X$.

\end{definition}

\begin{theorem}\label{CtyThm} Let $X$ and $Y$ be topological spaces and $f: X \to Y$ be a function. If $f$ is continuous then it is $T_1$ continuous. Furthermore, if $Y$ is $T_1$ then if $f$ is $T_1$ continuous it is also continuous. In particular, when $X$ and $Y$ are $T_1$, $f$ is continuous if and only if it is $T_1$ continuous.
\end{theorem}
\proof Suppose $f$ is continuous. Let $\mathcal{U}$ be an open cover of $Y$. Then $\mathcal{V}=\{f^{-1}(U) \mid U \in \mathcal{U} \}$ is an open cover of $X$ which meets the requirements. (Indeed, fix $x \in X$ and pick any $y \in X$. If there exists $V \in \mathcal{V}$ with $x,y \in V$ then $V=f^{-1}(U)$ for some $U \in \mathcal{U}$. Therefore $f(x),f(y) \in U$.)

Now suppose that $f$ is $T_1$ continuous and that $X$ and $Y$ are both $T_1$. (We will use the property that a function $f\colon X \to Y$, between any topological spaces $X$ and $Y$, is continuous at $x \in X$ if and only if for any net $(x_\lambda)_{\lambda \in \Lambda}$ with $\lim x_\lambda=x$, we have $\lim f(x_\lambda)=f(x)$.) Pick $x \in X$. Let $\varphi \colon \Lambda \to X$ be a net converging to $x \in X$. Write $\varphi = (x_\lambda)_{\lambda \in \Lambda}$. Let $U \ni f(x)$ be open. Let $\mathcal{U}$ be an open cover of $Y$ such that $U \in \mathcal{U}$ and for any $W \in \mathcal{U}$ with $W \neq U$, $f(x) \notin W$. Such an open cover exists as $Y$ is $T_1$. Then there exists an open cover $\mathcal{V}$ of $X$ such that for any $y \in X$, if there exists $V \in \mathcal{V}$ with $x,y \in V$ then there exists $W\in \mathcal{U}$ with $f(x),f(y) \in W$. Let $V \in \mathcal{V}$ such that $x \in V$ (in case of multiple such sets, just pick one). Then since $\lim x_\lambda = x$ there exists $\alpha \in \Lambda$ such that for any $\beta \geq \alpha$, $x_\beta \in V$. Then for any $\beta \geq \alpha$ there exists $U_\beta \in \mathcal{U}$ such that $f(x_\beta), f(x) \in U_\beta$. Since there is a unique element of $\mathcal{U}$ containing $f(x)$, i.e. $U$, this means $U_\beta=U$ for all $\beta \geq \alpha$; i.e. $f(x_\beta) \in U$ for all $\beta \geq \alpha$. Since $U$ was an arbitrarily picked open neighbourhood and we have shown $f(x_\lambda)$ is eventually in $U$, it follows that $\lim f(x_\lambda)=f(x)$ and so $f$ is continuous at $x$. Since $x \in X$ was picked arbitrarily we have that $f$ is continuous at all $x \in X$ and is thereby continuous.
\qed

\begin{lemma}\label{CtyLemma} A function $f \colon X \to Y$ is $T_1$ continuous at $x \in X$ if and only if for any open cover $\mathcal{U}$ of $Y$ and for any $n \in \mathbb{N}$ there exists an open cover $\mathcal{V}$ of $X$ such that for any $y \in X$, if there exists $V \in \mathcal{V}$ with $x,y \in V$ then for each $i \in \{0,1,\ldots, n\}$ there exists $U_i \in \mathcal{U}$ with $f^i(x),f^i(y) \in U_i$.
\end{lemma}

\proof
Clearly if the latter is true then the function is $T_1$ continuous. Thus, suppose that $f$ is $T_1$ continuous. Pick $x \in X$. Let $\mathcal{U}$ be given and let $n \in \mathbb{N}$. Let $\mathcal{V}_1$ be an open cover corresponding to $\mathcal{U}$ and $f^{n-1}(x)$ as in $T_1$ continuity. Notice that, without loss of generality, $\mathcal{V}_1$ refines $\mathcal{U}$ (we can take the open cover given by the union of all pairwise intersections of each element of $\mathcal{U}$ with each element of $\mathcal{V}$). Now let $\mathcal{V}_2$ refine $\mathcal{V}_1$ correspond to $\mathcal{V}_1$ and $f^{n-2}(x)$ as in $T_1$ continuity. Continuing in this way, and defining $\mathcal{V}_0\coloneqq \mathcal{U}$, we obtain a refining sequence of open covers
\[\mathcal{V}_0=\mathcal{U},\mathcal{V}_1,\mathcal{V}_2 , \ldots , \mathcal{V}_n,\]
such that for all $i \in \{1,\ldots,n\}$ and for any $y \in X$, if there exists $V_i \in \mathcal{V}_i$ with $f^{n-i}(x),y \in V_i$ then there exists $V_{i-1} \in \mathcal{V}_{i-1}$ with $f^{n-i+1}(x),f(y) \in V_{i-1}$. Thus, by construction, $\mathcal{V}_{n}$ corresponds to $\mathcal{V}_{n-1}$ and $f^0(x)=x$. Now consider $\mathcal{V}_n$ pick $y \in X$. Suppose there exists $V_n \in \mathcal{V}_n$ such that $x,y \in V_n$ (otherwise we are done). Then there exists $V_{n-1} \in \mathcal{V}_{n-1}$ such that $f(x),f(y) \in V_{n-1}$. Then, by construction, there exists $V_{n-2} \in \mathcal{V}_{n-2}$ such that $f^2(x),f^2(y) \in V_{n-2}$; indeed, for each $i \in \{0,1,\ldots,n\}$, there exists $V_{n-i} \in \mathcal{V}_{n-i}$ such that $f^i(x),f^i(y) \in V_{n-2}$. But since $\mathcal{V}_i$ is a refinement of $\mathcal{U}$ for all $i \in \{0,\ldots, n\}$ the result follows.
\qed


==> EqAndChaos/3.Minimal.tex <==
\subsection{Minimal systems}

For a minimal system, the following is the Auslander-Yorke Dichotomy Theorem \cite{AuslanderYorke}.

\begin{theorem} A minimal system is either equicontinuous or sensitive.
\end{theorem}

If a compact metric system has a dense set of minimal points, we have that if it is sensitive it is also syndetically sensitive with the same constant of sensitivity \cite{Moothathu}; this generalises to compact Hausdorff systems. Using this fact, the above dichotomy becomes:

\begin{corollary} A minimal system is either equicontinuous or syndetically sensitive.
\end{corollary}

Akin {\em et al} \cite{AkinAuslanderBerg} show that if $\Eq(X,f) \neq \emptyset$ and the system is minimal then it is equicontinuous. We can extend this to: if $\EP(X,f)\neq \emptyset$ and the system is minimal then it is equicontinuous. Indeed, a point $x$ in a minimal system has an equicontinuity partner if and only if it is an equicontinuity point. *WHY???*
%Why is this true?? 
We may then write:
 
 \begin{corollary} A minimal system is either equicontinuous or there are no equicontinuity pairs and the system is syndetically sensitive.
 \end{corollary}
 
We close this modest section with the following straightforward result.
 
\begin{proposition} A dynamical system $(X,f)$ has a syndetically transitive point $x \in X$, i.e. there exists $x \in X$ such that, for any nonempty open $U$, $N(x,U)$ is syndetic, if and only if the system is minimal; in which case every point is syndetically transitive.
\end{proposition}

\proof 
Suppose $(X,f)$ is minimal. Pick $x \in X$. Then $x$ is a minimal point. Let $U$ be nonempty open. Pick $a \in U$ such that $a=f^n(x)$ for some $n\in \mathbb{N}$; since $x$ is transitive such a point exists. Then $N(a,U)$ is syndetic as $a$ is a minimal point and $U$ is a neighbourhood of it. Since $a \in \Orb(x)$ it follows that $N(x,U)$ is syndetic. Therefore, as $x$ was picked arbitrarily, every point is a syndetically transitive point.

Now suppose $x\in X$ is a syndetically transitive point. Then $N(x,U)$ is syndetic for any open $U \ni x$; this implies $x$ is minimal. Therefore $\omega (x)=X$ is a minimal set; $(X,f)$ is minimal. The fact that every point is transitive now follows from the previous part.
\qed
 
%The following question is of interest: Under what conditions does the absence of any equicontinuity pairs imply regular-chaos? As mentioned (Proposition \ref{prop}), the converse is always true.
 
 %(QUESTION: Does regular-chaos entail some kind of regularity?)

==> EqAndChaos/4.OROC.tex <==
\subsection{Other results on chaos}

Let $P$ and $Q$ be properties that may be exhibited by certain subsets of $\mathbb{N}$, themselves with the following properties:
\begin{enumerate}
\item If $A \subseteq \mathbb{N}$ satisfies $P$ (resp. $Q$), and $B \supseteq A$, then $B$ satisfies $P$ (resp. $Q$).
\item If $A\subseteq \mathbb{N}$ satisfies $P$ (resp. $Q$), then for any $k \in \mathbb{N}$, $A\setminus \{0,1,2,\ldots,k\}$ satisfies $P$ (resp. $Q$).
\item If $A \subseteq \mathbb{N}$ satisfies $P$ and $B \subseteq \mathbb{N}$ satisfies $Q$ then $A \cap B \neq \emptyset$.
\end{enumerate}

Examples of such pairs of properties are:
\begin{enumerate}
\item $P =$ syndetic, $Q=$ thick. (and vice-versa.)
\item $P=$ infinite, $Q=$ cofinite.
\item $P=IP^*$, $Q=IP$.\footnote{Recall, a set of natural numbers is called an $IP$-set if it contains all finite sums of some subsequence of itself (when viewing the set as a sequence). An $IP^*$-set is one which has non-empty intersection with any $IP$-set. See \cite{Bergelson} for more information. }
\end{enumerate}

We have the following sufficient condition for a system being $P$-sensitive; this condition generalises one given in \cite{Moothathu} for syndetic sensitivity. Throughout this section $X$ is a compact Hausdorff space.

\begin{proposition}\label{Prop2} Let $(X,f)$ be a dynamical system. Suppose that for any nonempty open pair $U$ and $V$, $N(U,V)$ satisfies $P$. Suppose there exists a set $A$ satisfying $Q$, where $Q$ has the previously mentioned properties, such that there exists a symmetric $D \in \mathscr{D}$ such that for any $n\in A$ there exists $x \in X$ with $(x, f^n(x)) \notin D$. Then for any nonempty open $U$, $N_D(U)$ satisfies $P$; so $(X,f)$ is $P$-sensitive, with sensitivity entourage $D$.
\end{proposition}

\proof
Let $U \subseteq X$ be nonempty open. Since $N(U,U)$ is $P$, and $A$ is $Q$, there exists $n \in N(U,U) \cap A$. Define $W \coloneqq U \cap f^{-n}(U)$; then $W$ is nonempty open. Since $n \in A$ there exists $x \in X$ with $(x,f^n(x))\notin D$. Let $V \ni x$ be open such that if $y \in V$ then $(y, f^n(y)) \notin D$; such a set exists by continuity of $f$. Now consider the $P$-set $N(W,V)$; we will show $N(W,V) \subseteq N(U, D)$, from which it will follow that $N_D(U)$ is $P$. Let $m \in N(W,V)$ and let $w \in W \subseteq U$ be such that $f^m(w) \in V$. Then $(f^m(w),f^{m+n}(w)) \notin D$ by our choice of $V$. Let $u=f^n(w) \in U$; then $(f^m(w), f^m(u)) \notin D$, so $m \in N_D(U)$.
\qed

This result yields a corollary relating to recurrence which also follows as an implicit corollary from several results in \cite{AkinAuslanderBerg}. %RIGIDITY IN AKIN PAPER IMPLIES THIS (Trans + almost eq gives uniformly rigid. Plus Trans + Eq=\emptyset implies  sensitive . Thus: non-recurrent \implies not uniformly rigid \implies (not trans OR not a.e.); since trans therefore not a.e., therefore sensitive. - cite that it follows as a corollary from this paper.

\begin{corollary}\label{cor4.0} If a system $(X,f)$ is topologically transitive an has a non-recurrent point then it is sensitive.
\end{corollary}

\proof For a non-recurrent point $x \in X$, there exists a cofinite set $A$ and an entourage $D \in \mathscr{D}$ such that $f^n(x) \notin D[x]$ for any $n \in A$. Applying Proposition \ref{Prop2} gives the result.
\qed

\begin{corollary}\label{cor4.1}
Let $(X,f)$ be a transitive system. If $\bigcup_{x \in X} \omega(x) \neq X$ then the system is sensitive. 
\end{corollary}

\proof 
Follows immediately from Corollary \ref{cor4.0}. (Of course, for systems with a transitive point this is vacuous.)
\qed


%The following is wrong

%\begin{corollary} If a system $(X,f)$ is thickly transitive and non-minimal then it is thickly sensitive.
%\end{corollary}

%\proof
%Let $x \in X$ be a non-minimal point. Then there exists a neighbourhood $U$ of $x$ such that $N(x,U)$, the set of return times of $x$ to $U$, is not syndetic.\footnote{It is folklore that a point $x$ in a compact Hausdorff system is minimal if and only if $N(x,U)$ is syndetic for every neighbourhood $U$ of $x$.} Let $D \in \mathscr{D}$ be symmetric such that $D[x] \subseteq U$. Then let $A=N(x, D[x])$. For any $n \in A$ .... Actually we need $\mathbb{N}\setminus N(x,U)$ to be syndetic (i.e. x is syndetically not close to itself.... But if x is recurrent this will not be the case; we could use continuity to make iterates of x stay close to x... wait no that's not right (it'd stay close to the first n iterates of x). So there may be some instances where every point is recurrent but this result holds.



\begin{corollary} Let $(X,f)$ be a $P$-transitive system. Suppose that there exists two distinct points $x,y \in X$ and a $Q$-set $A=\{n_k \mid k \in \mathbb{N}\}$ such that for any symmetric $D \in \mathscr{D}$, there exists $l \in \mathbb{N}$ such that $(f^{n_k}(x),f^{n_k}(y)) \in D$ for all $k \geq l$. Then $f$ is $P$-sensitive.
\end{corollary}

\proof
Choose $D \in \mathscr{D}$ such that $3D \not\ni (x,y)$. Let $l \in \mathbb{N}$ be such that $(f^{n_k}(x),f^{n_k}(y)) \in D$ for all $k \geq l$. Then, for any $k \geq l$, either $(x,f^{n_k}(x)) \notin D$ or $(y, f^{n_k}(y)) \notin D$. Indeed, suppose that both are in $D$. Then by the triangle inequality, used twice, $(x,y) \in 3D$; a contradiction. Now take $B=\{ n_k \mid k \geq l \}$; $B$ is a $Q$-set, therefore by Proposition \ref{Prop2} we are done.
\qed

We emphasise the following corollary, particularly the fact that a transitive system which is not injective is sensitive; however this is known (see, for example, \cite[pp ~.335]{deVries}.)

\begin{corollary} Let $(X,f)$ be a dynamical system.
\begin{enumerate}
\item If $(X,f)$ is $P$-transitive and not injective then it is $P$-sensitive.
\item If $(X,f)$ is syndetically transitive and not injective it is syndetically sensitive.
\item If $(X,f)$ is thickly transitive and not injective it is thickly sensitive.
\item If $(X,f)$ is transitive and not injective then it is sensitive.\footnote{This result holds because saying for all nonempty open pairs $N(U,V) \neq \emptyset$ is equivalent to saying $N(U,V)$ is infinite for all such pairs. Therefore, $P$ meaning, ``Is nonempty", is equivalent (in this case) to $P$ meaning, ``Is infinite".}
\end{enumerate}
\end{corollary}

%\subsection{A note on shadowing and chaos}
%It is easy to show that if a system exhibits shadowing then it is topologically transitive if and only if it is chain transitive.

==> EqAndChaos/7.SpacesAdTrans.tex <==
\section{Spaces admitting transitive maps}

It is well-known that if a space $X$ has a finite open set then any transitive map on $X$ consists of a single periodic orbit.\footnote{The space $X$ need not be Hausdorff; this holds for an arbitrary topological space.} Thus, a necessary condition for an infinite Hausdorff space to admit a transitive map is that it be perfect. Generally, one can ask what kind of spaces admit such maps. See for example \cite{NagarKannan}, where the authors show what subspaces of $\mathbb{R}$ admit transitive maps. We assume the following theorem is known, however we have not ourselves seen it expressed. In any case, it is worth expressing.

\begin{theorem} Let $X$ be a $T_1$ topological space. If $X$ admits a transitive map then either every nonempty open subset has the same density or the space is finite. 
\end{theorem}

\begin{proof} As $X$ is $T_1$ if an open set is finite then every point in that set is isolated. Thus, if there exists a finite open set then any transitive map would consist of a single periodic orbit, meaning that $X$ is finite.

Now suppose that $X$ has no isolated points. Let $U$ be nonempty open, with least density $\kappa$ (i.e. every open set has density at least $\kappa$). The continuous image of a set with density $\kappa$ has density at most $\kappa$; the union of a countable collection of subspaces, each with density at most $\kappa$, itself has density at most $\kappa$. Therefore for any continuous map $f\colon X \to X$, $\bigcup_{i=0} ^\infty f^i(U)$ has density at most $\kappa$; if $f$ is transitive then this set is dense in $X$ meaning $X$ has density at most $\kappa$. The result follows.
\end{proof}

\begin{corollary}
If $X$ has an nonempty open subset $U$ which is separable and $X$ admits a transitive map, then $X$ is separable.
\end{corollary}

From this is follows that, for example, there is no transitive map on the unit square with lexicographic ordering; this space is not separable but has separable nonempty open sets (see \cite[pp. ~73]{SteenSeebach}).

==> EqAndChaos/Appendices.tex <==
\section{Appendix}

\subsection{Uniform spaces}
\input{Preliminaries/Uniformities}







%This theorem can be found in \cite[S. 4.2]{W}.

%\begin{theorem}\label{A1}
%The neighbourhood system $\mathscr{U}_x$ at $x$ (i.e. the collection of all neighbourhoods of $x$) in a topological space $X$ has the following properties:
%\begin{enumerate}[label=\alph*).]
%\item If $U \in \mathscr{U}_x$, then $x \in U$,
%\item If $U, V \in \mathscr{U}_x$, then $U \cap V \in \mathscr{U}_x$,
%\item If $U \in \mathscr{U}_x$, then there is a $V \in \mathscr{U_x}$, such that $U \in \mathscr{U}_y$ for all $y \in V$,
%\item If $U \in \mathscr{U}_x$ and $U \subseteq V$, then $V \in \mathscr{U}_x$; and finally
%\item $G \subseteq X$ is open if and only if $G$ contains a neighbourhood of each of its points.
%\end{enumerate}
%Conversely, if for a set $X$, a collection $\mathscr{U}_x$ of subsets of $X$ is assigned to each $x \in X$ such that a)-d) are satisfied and if e) is used to define precisely when a subset of $X$ is declared open, the result is a topology on $X$ in which the neighbourhood system at $x \in X$ is precisely $\mathscr{U}_x$ for all $x \in X$.
%\end{theorem}

%\begin{definition} A set $A$ is said to be nowhere dense if $int(\overline{A})=\emptyset$.
%\end{definition}

%\begin{definition} A set is said to be meagre if it can be written as a countable union of nowhere dense sets. A set that is not meagre is said to be non-meagre (or of Baire second category).
%\end{definition}

%\begin{proposition} A topological space is non-meagre if and only if any countable intersection of dense open sets is nonempty. 
%\end{proposition}
%\proof
%We prove the left to right entailment here.

%Suppose $\{U_i\}_{i\geq1}$ is a countable collection of open dense sets. Then, for each $i$, $C_i =X \setminus U_i$ is closed and nowhere dense ($int(\overline{C_i})=int(C_i)=\emptyset$ (otherwise $U_i$ is not dense)). Then clearly
%\[ \bigcap_{i \geq 1} U_i = X \setminus \bigcup_{i\geq 1} C_i.\]
%But $\bigcup_{i\geq 1} C_i \subsetneq X$, since if $\bigcup_{i\geq 1} C_i=X$ then $X$ would be meagre. Therefore $X \setminus \bigcup_{i\geq 1} C_i \neq \emptyset$, and so $\bigcap_{i \geq 1} U_i \neq \emptyset$.
%\qed

%\begin{definition} A $\pi$-base for a topological space $X$ is a collection $\mathscr{U}$ of nonempty open sets in $X$ such that if $R$ is any nonempty open set in $X$ then there exists $V \in \mathscr{U}$ such that $V \subseteq R$.
%\end{definition}

%\begin{definition} A density basis for a topological space $X$ is a collection $\mathscr{V}$ of nonempty open sets in $X$ such that if $A \subseteq X$ is such that $A \cap V \neq \emptyset$ for any $V \in \mathscr{V}$, then $\overline{A}=X$.
%\end{definition}

%We prove that the notions of density basis and $\pi$-base are equivalent.

%\begin{proposition} Let $X$ be a topological space. A collection is a $\pi$-base if and only if it is a density basis.
%\end{proposition}


==> EqAndChaos/Questions.tex <==
\subsection{Questions}
We end this section on chaos with some questions for further exploration.


\begin{enumerate}
\item Does transitivity and sensitivity entail some form of regularity? %(NB. de Vries book has some examples showing transitivity and sensitivity does not entail dense periodic points. Have a look at these examples to see if they do have some regularity in common.) 
\item Does full-chaos entail some kind of regularity?
%\item Moothathu \cite{Mooth} (originally defines in an earlier paper - CITE) defines {\em multi-transitivity}: $(X,f)$ is said to be multi-transitive if $f \times f^2 \times \cdots \times f^m : X^m \to X^m$ is transitive for every $m \in \mathbb{N}$. For compact minimal systems multi-transitivity is equivalent to weak mixing but in general there are no implications between them \cite{Mooth}. - Look in to. 

%Also, weak-mixing can be extended to a finite product being transitive. If any finite product is transitive then it would follow that that system is thickly transitive ? (I think...)
\end{enumerate}

As previously mentioned, when Devaney first defined what we now call Devaney-chaos, he referred to the dense set of periodic points as ``an element of regularity," in the midst of random behaviour \cite{Devaney}. It would be interesting to see if fully-chaotic systems do necessarily exhibit some element of regularity.

*LOOK AT THIS AND ADJUST ACCORDINGLY*

==> Preliminaries/Uniformities.tex <==
%\section{Uniform Spaces}

The definitions in this section can be found in \cite{Willard}. Let $X$ be a set. The diagonal of the Cartesian product $X \times X$ is the set $\Delta=\{(x,x) \mid x \in X \}$. Given two subsets $A$ and $B$ of $X \times X$, we define the composition of these sets as $A \circ B = \{(x,z) \mid \text{there exists } y \in X \text{ such that } (x,y) \in B \text{ and } (y, z) \in A\}$. We write $nA$ to denote $\underbrace{A \circ A\circ \ldots \circ A}_{n \text{ times}}$. We define the inverse $A^{-1}=\{(x,y) \mid (y,x) \in A \}$. If $A \subset X \times X$ contains the diagonal $\Delta$ we say it is an {\em entourage of the diagonal}.

\begin{definition} A uniformity $\mathscr{D}$ on a set $X$ is a collection of entourages of the diagonal such that the following conditions are satisfied.

\begin{enumerate}[label=\alph*.]
\item $D_1, D_2 \in \mathscr{D} \implies D_1 \cap D_2 \in \mathscr{D}$.
\item $D \in \mathscr{D}, D \subset E \implies E \in \mathscr{D}$.
\item $D \in \mathscr{D} \implies E \circ E \subset \mathscr{D}$ for some $E \in \mathscr{D}$.
\item $D \in \mathscr{D} \implies E^{-1}\subset D$ for some $E \in \mathscr{D}$.
\end{enumerate}

\end{definition}

We call the pair $(X, \mathscr{D})$ a {\em uniform space}. We say $\mathscr{D}$ is {\em separating} if $\bigcap_{D \in \mathscr{D}} D = \Delta$; in this case we say $X$ is {\em separated}. A subcollection $\mathscr{E}$ of $\mathscr{D}$ is said to be a {\em base} for $\mathscr{D}$ if for any $D \in\mathscr{D}$ there exists $E \in \mathscr{E}$ such that $E \subset D$. Clearly any base $\mathscr{E}$ for a uniformity will have the following properties:
\begin{enumerate}
\item $D_1, D_2 \in \mathscr{D} \implies$ there exists $ E \in \mathscr{E}$ such that $ E \subseteq D_1 \cap D_2 $.
\item $D \in \mathscr{D} \implies E \circ E \subset \mathscr{D}$ for some $E \in \mathscr{D}$.
\item $D \in \mathscr{D} \implies E^{-1}\subset D$ for some $E \in \mathscr{D}$.
\end{enumerate}
If $\mathscr{D}$ is separating then $\mathscr{E}$ will satisfy $\bigcap_{E \in \mathscr{E}} E = \Delta$. A {\em subbase} for $\mathscr{D}$ is a subcollection such that the collection of all finite intersections from said subcollection form a base. We say an entourage of the diagonal $D$ is {\em symmetric} if $D=D^{-1}$.

\begin{remark} The symmetric sets in a uniformity $\mathscr{D}$ form a base for said uniformity.
\end{remark}

\begin{remark} If $D \in \mathscr{D}$ then $D^{-1} \in \mathscr{D}$, for any uniformity $\mathscr{D}$ on $X$.
\end{remark}

For an entourage $D \in \mathscr{D}$ and a point $x \in X$ we define the set $D[x]= \{y \in X \mid (x,y) \in D\}$. This naturally extends to a subset $A \subseteq X$; $D[A]= \bigcup_{x \in X}D[x]$. The following result can be found in \cite[Section 35.6]{Willard}.
\begin{theorem} \leavevmode
\begin{enumerate}[label=\alph*).]
\item For all $x \in X$, the collection $\mathscr{U}_x \coloneqq \{ D[x] \mid D \in \mathscr{D} \}$ is a neighbourhood base at $x$, making $X$ a topological space. The same topology is produced if any base $\mathscr{E}$ of $\mathscr{D}$ is used in place of $\mathscr{D}$.
\item The topology is Hausdorff if and only if $\mathscr{D}$ is separating.
\end{enumerate}
\end{theorem}
Note that, by \cite[Section 25.6]{Willard}, for any $x \in X$, the collection $\mathcal{U}_x = \{D[x] \mid D \in \mathscr{D} \}$ forms a neighbourhood basis at $x$; in particular $D[x]$ is a neighbourhood of $x$ for any $D \in \mathscr{D}$. 

Finally we remark that for a compact Hausdorff space $X$, by \cite[Section 8.3.13]{Engelking}, there is a unique uniformity $\mathscr{D}$ which induces it. The entourages in this uniformity are all neighbourhoods of the diagonal $1_X$. Given an open cover of $X$, say $\mathcal{U}$, the set $D \subset X \times X$ defined by $(x,y) \in D$ if and only if there exists $U \in \mathcal{U}$ such that $x,y \in U$ is an entourage in the uniformity.

In general, a cover of a uniform space $(X, \mathscr{D})$ is a {\em uniform cover} if and only if it is refined by a cover of the form $\mathcal{U}_D=\{D[x] \mid x \in X\}$ for some $D \in \mathscr{D}$.
